HaliVer: Deductive Verification and Scheduling Languages Join Forces

The HaliVer tool integrates deductive verification into the popular scheduling language Halide, used for image processing pipelines and array computations. HaliVer uses Vercors, a separation logic-based verifier, to verify the correctness of (1) the Halide algorithms and (2) the optimised parallel code produced by \halide when an optimisation schedule is applied to the algorithm. This allows proving complex, optimised code correct while reducing the effort to provide the required verification annotations. For both approaches, the same specification is used. We evaluated the tool on several optimised programs generated from characteristic Halide algorithms, using all but one of the essential scheduling directives available in Halide. Without annotation effort, Haliver proves memory safety in almost all programs. With annotations Haliver, additionally, proves functional correctness properties. We show that the approach is viable and reduces the manual annotation effort by an order of magnitude.

==> src/annotations.tex <==
\section{Adding \& Transforming Annotations}\label{sec:annotations}
\subsection{Adding Annotations}\label{sec:adding}
% What kind of annotations do we add
We add verification annotations to the algorithm part of the Halide language to verify Halide programs. Intuitively, the verification annotations act similar to Hoare logic. We write an assertion of the form $\hoare{P} S \hoare{Q}$ to indicate that if pre-condition $P$ holds in the initial state of the program, then post-condition $Q$ holds in the state we end up after executing $S$.\footnote{Since the Halide algorithm language does not include recursion or arbitrary loops, all Halide programs will always terminate. Therefore, we do not add a terminating requirement here.} \todo{Should I say more about "state", what is state means in this Halide context (I'd say the state contains input, parameters and functions, and each function contains values for specific input points)}

In Fig. \ref{fig:syntax-annotations} we add the specific locations where annotations can be added in the Halide syntax, and the correspondence is that with $\hoare{P} S \hoare{Q}$ is that $S$ is equivalent to a pipeline. Around each function definition, annotations can be placed, to check intermediate states. One must add \textit{reduction invariant} annotations to reduction domains ($R$) to help prove a program correct. Intuitively, a reduction invariant is similar to a loop invariant. It must hold before the reduction starts and it must be preserved during each step of the reduction. Lastly, afterwards, it should, after each reduction variable has reached its maximum value, imply any post-conditions we are interested in.

\begin{figure}
\centering
\begin{tabular}{lcll}
\hline
$R$ & $::=$ & $\rdom{r_1 = I_1, \hoare{A_{inv_{r1}}}; \cdots ; r_n = I_n, \hoare{A_{inv_{rn}}}}{e}$ & Reduction domain \\
$U_0$ & $::=$ & $\hoare{A_{pre}} e \hoare{A_{post}}$ & Pure stage \\
$U$ & $::=$ & $ \hoare{A_{pre}} R \mathbf{~in~} (e_1, \ldots , e_n) \leftarrow e \mathbf{~if~} e_P \hoare{A_{post}}$ & Update stage \\
$B$ & $::=$ & $U_0 ~\vbar~ B;U$ & Function body \\
$F$ & $::=$ & $\fun f (x_1, \dots , x_n) = \{B\}$ & Function \\
$D$ & $::=$ & $F ~\vbar~ D; F$ & Definitions \\
$P$ & $::=$ & $\hoare{A_{pre}} \pipeline(p_1, \ldots , p_m, b_1, \ldots , b_k) = D \hoare{A_{post}}$ & Pipeline \\
\hline
$A$ & $::= $ & $e$ & Annotation\\
\hline
$c$ & $::=$ & $i \in \mathbb{V}$ & Constants \\
$a$ & $::=$ & $f[e_1, \ldots, e_n]$ & Func access \\
$i$ & $::=$ & $b[e_1, \ldots, e_n]$ & Buffer access \\
$e$ & $::=$ & $c~\vbar~a~\vbar~v~\vbar~\mathbf{op}(e_1, \ldots, e_k)$ & Expression\\
$I$ & $::=$ & $(e_{min}, e_{len})$ & Interval \\
$v$ & $::=$ & $x$ & Pure variable \\
    & $\vbar$ & $r$ & Reduction variable \\
    & $\vbar$ & $p$ & Parameter variable \\
$\mathbf{op}$ & $::=$ & $x$ & Pure variable \\
\hline
$Z$ & $::= $ & $P(z)$ & Realization \\
$z$ & $::=$ & $ \langle (I_1, \ldots , I_n), (c_1, \ldots , c_m), (b_1, \ldots , b_k) \rangle $ & Input \\
$b$ & & & Input buffer \\
\hline
\end{tabular}
\caption{\label{fig:syntax-annotations}Halide algorithm syntax, retrieved from \cite[Figure 4 and 5]{reinkingFormalSemanticsHalide2020}, but altered to add annotations points ($A$) and input buffers ($b$). \todo{Unsure about using name $b$ for input buffer, and especially the line with $P$ and $z$, where I both use $b$}}
\end{figure}

Function definition annotations can only refer to their own function point-wise since functions are defined pointwise. I.e. for function \lstinline|f(x,y)| we can refer to \lstinline|f(x,y)| and no other points for function \lstinline|f|. It is allowed to call other functions in the annotations. Thus \lstinline|f.requires(f(x,y) == g(0,1))| is allowed, but \lstinline|f.requires(f(x,y) == f(0,1))| is not. As a shorthand for the own function we defined, we use the notation \lstinline|\result|, as it equivalent to the resulting value of the function or the pointwise value of the input.

\todo{I'm unsure about these examples and what kind of format I should use them (and if they are needed at all). Below is the 'code' format, which is more readable I think. But 'formal' syntax is used in Fig. \ref{fig:syntax-annotations}, which is easier to use later on if I want to describe transformations/translations. What do you think?}
Consider the example below, where we require as a pre-condition that the input is between the values $0$ and $255$.
\begin{lstlisting}
Func blur(Buffer<int> input){
  Var x, y;
  Func blur_x, blur_y;
  input.requires(\result >= 0 && \result <= 255);

  blur_x(x,y) = (input(x-1,y) + input(x,y) + input(x+1,y))/3
  blur_x.ensures(\result >= 0 && \result <= 255);

  blur_y(x,y) = (blur_x(x,y-1) + blur_x(x,y) + blur_x(x,y+1))/3;
  blur_y.ensures(\result >= 0 && \result <= 255);

  return blur_y;
}
\end{lstlisting}
The \lstinline|\result| indicates the value of functions and input at their standard arguments (e.g. \lstinline|blur_x(x,y)|). The annotation for \lstinline|blur_x| is not needed to verify this example, but can be useful to check intermediate conditions.

We could write the same example, but using a reduction domain. Now we would use a reduction invariant, this looks like.
\begin{lstlisting}
Func blur(Buffer<int> input){
  Var x, y;
  Func blur;
  Rdom r(-1,3,-1,3);
  input.requires(\result >= 0 && \result <= 255);

  blur(x,y) = 0;
  blur(x,y) += input(x+r.x,y+r.y);
  blur.invariant(\result >= 0 && \result <= 255 * 9);
  blur(x,y) = blur(x,y)/9;
  blur.ensures(\result >= 0 && \result <= 255);

  return blur;
}
\end{lstlisting}

\subsubsection{Semantics}
% Semantics of Annotations

\subsubsection{Translating to Prototype Verification Language}
% How we translate to PVL code

In Fig. \ref{fig:translate} we show how the front end of Halide can be directly translated to PVL, which VerCors can directly use to verify the code. Intuitively, the following happens:
\begin{enumerate}
\item[\textbf{Input buffers:}] Gets translated as an abstract function, any pre-conditions concerning the input buffer, is a post-condition of this abstract function.
\item[\textbf{Function:}] Each function gets translated into subfunctions, each definition $U_i$ gets its own function in PVL, and the complete function calls the subfunction from the last definition.
\item[\textbf{Pure Definition:}] Gets translated as is.
\item[\textbf{Update Definition:}] The conditions of the update definition are checked, if true, go to the body of the function, otherwise call the previous defined subfunction. Any calls to the function are replaced by the previous defined subfunction.
\item[\textbf{Reduction Update:}] In essence we use recursion to model reduction, and the reduction variables are given as explicit parameters to the translated recursive function. Any call to the function is replaced by the call to the recursive function, but with the reduction variable decreased by one. If the reduction variable is equal to the minimum value, the function represents the state of the function before the reduction has begun. If the the reduction variable has value $i$ then the recursive function represents the state of the original function after the reduction variable had value $i-1$ and the body was executed. Any reduction invariants are given as ensure annotations to the recursive function. With multiple reduction variables, multiple recursive functions are made, one for each reduction variable.
\end{enumerate}



 We show how functions get translated, expressions are translated in the regular way you would expect, e.g. $x+y$ in Halide is still $x+y$ in PVL. Only expression which divide are replaced by a guard, since Halide defines dividing by zero as being equal to one. \todo{Or it was zero, I have to look this up, it is in the master thesis about Halide semantics}.

\begin{figure}
\centering
\line(1,0){\textwidth}\\
Input buffer transformation \\
We model buffer $b$ of type $t$, with any requirements on the buffer given by annotation $p$, with dimensionality $n$ as an abstract function in PVL. It has no body, but it adheres to the annotations given to it.

$\downarrow$ \\
\begin{lstlisting}[frame=none,numbers=none]
  ensures p;
pure t b(int x1, ..., int xn);
\end{lstlisting}
\line(1,0){\textwidth}\\
Whole function transformation \\
$\fun f (x_1, \dots , x_n) = \{U_0; \cdots U_k \}$\\

$\downarrow$ \\
\begin{lstlisting}[frame=none,numbers=none]
pure t f(int x1, ..., int xn) = fk(x1, ..., xn)
\end{lstlisting}
where $t = \toT{U_0}$ \\
\line(1,0){\textwidth}\\

Pure definition transformation \\
$\fun f (x_1, \dots , x_n) = \{U_0; \cdots U_k \}$ \\
where $U_0 = \hoare{Q}e_b\hoare{P}$ \\
$\downarrow$ \\
\begin{lstlisting}[frame=none,numbers=none]
  requires q;
  ensures p;
pure t f0(int x1, .., int xn) = eb;
\end{lstlisting}
where $t = \toT{U_0}$, $eb = \toE{e_b}$, $q = \toE{Q}$ and $p = \toE{P}$
\line(1,0){\textwidth}\\
Update definition (Empty reduction domain) \\
$\fun f (x_1, \dots , x_n) = \{\cdots ; U_i; \cdots\}$ \\
where $U_i = \hoare{Q}\rdom{} (e_1, \ldots , e_n) \leftarrow e_b \mathbf{~if~} e_P \hoare{P}$ \\
$\downarrow$ \\
\begin{lstlisting}[frame=none,numbers=none]
  requires q;
  ensures p;
pure t t fi(int x1, .., int xn) = x1==e1 && .. && xk==en && ep ?
  eb : fprev(x1, .., xk);
\end{lstlisting}
where $t = \toT{U_0}$, $e1= \toE{e_1}$, ... , $ek= \toE{e_k}$, $eb = \toE{e_b}$, $ep = \toE{e_p}$, $q = \toE{Q}$, $p = \toE{P}$  and \lstinline|fprev| is the previous function stage. E.g. when defining \lstinline|f4| the previous stage is \lstinline|f3|.\\
% $\fun f (x_1, \dots , x_n) = \{\cdots ; U_i; \cdots\}$ & \lstinline|  ensures p;|\\
% $U_i = \hoare{Q}\rdom{} (e_1, \ldots , e_n) \leftarrow e \mathbf{~if~} e_P \hoare{P}$  & \lstinline|pure t fi(int x1, ..., int xn) =|
% \\
% & \lstinline|  x1 == e1 && ... && xk == en && ep ? eb | \\
% & \lstinline|    : fprev(x1, ..., xk)|\\
% & where $t = \toT{U_0}$, $e1= \toE{e_1}$, ... , $ek= \toE{e_k}$, $eb = \toE{e_b}$,\\ & $ep = \toE{e_p}$, $q = \toE{Q}$, $p = \toE{P}$  and $fprev$ is the previous \\ & function stage. E.g. when defining $f4$ the previous \\
% & stage is $f3$.\\ \hline

\line(1,0){\textwidth}\\
\caption{\label{fig:translate} Rules for translating Halide algorithm code towards PVL.}
\end{figure}
\begin{figure}
\ContinuedFloat
\line(1,0){\textwidth}\\
\centering
Update definition (with reduction domain) \\
$\fun f (x_1, \dots , x_n) = \{\cdots ; U_i; \cdots\}$ \\
$U_i = \hoare{Q}\mathbf{rdom} (r_1 = (e_{min_{1}}, e_{len_1}), \hoare{I_{r_1}}; \cdots ; r_k = (e_{min_k}, e_{len_k}), \hoare{I_{r_{k}}}) \mathbf{~in~ }(e_1, \ldots , e_n) \leftarrow e_b \mathbf{~if~} e_P \hoare{P}$

$\downarrow$ \\
\begin{lstlisting}[frame=none,numbers=none]
  requires q;
  ensures p;
pure t fi(int x1, .., int xn) = fi_rk(x1, .., xn, emax_k);

  requires emin_k <= rk && rk <= emax_k;
  ensures ik;
pure t fi_rk(int x1, .., int xn, int rk) =
  rk == emin_k ? fi1(x1, .., xn) : fi_rk1(x1, .., xn, emax_k1, rk-1);

..

  requires emin_k <= rk && rk < emax_k;
  ..
  requires emin_2 <= rk && rk <= emax_2;
  ensures i2;
pure t fi_r2(int x1, .., int xn, int r2, ..., int rk1, int rk) =
  r2 == emin_2 && .. && rk == emin_k ? fi1(x1, .., xn)
    : r2 == emin_2 && .. && rk1 == emin_k1
      ? fi_r2(x1, .., xn, emax2, ..,emax_k1 , rk-1)
      : ..
      ..
        : fi_r1(x1, .., xn, emax1, r2-1, .., rk);

  requires emin_k <= rk && rk < emax_k;
  ..
  requires emin_1 <= rk && rk <= emax_1;
  ensures i1;
pure t fi_r1(int x1, ..., int xn, int r1, ..., int rk1, int rk) =
  r2 == emin_2 && .. && rk1 == emin_k1 && rk == emin_k ? fi1(x1, .., xn)
    : r2 == emin_2 && .. && rk1 == emin_k1
      ? fi_r2(x1, .., xn, emax2, .., rk-1)
      : ..
      ..
        : x1 == e1 && .. && xn == en && ep ?
          ? eb
          : fi_r1(x1, .., xn, r1-1, .., rk);
\end{lstlisting}
where \lstinline|fi1| refers to the translated function definition of $U_{i-1}$, $\mathtt{t} = \toT{U_0}$, $\forall j \in[1,n] . \mathtt{ej}= \toE{e_j}$, $\mathtt{eb} = \toE{e_b}$, $\mathtt{ep} = \toE{e_p}$, $\mathtt{q} = \toE{Q}$, $\mathtt{p} = \toE{P}$, $\forall l \in[1,k] . \mathtt{il} = \toE{I_{r_l}}$ , $\mathtt{emin_l} = \toE{e_{min_l}}$, $\mathtt{emax_l} = \toE{e_{min_l} + e_{len_l}}$.\\
And $\toE{\cdot}$ converts an expression to PVL, but additionally any occurrence of $r_1$ gets replaced by $r_1-1$ (\textbf{only} for $r_1$), and any mention of $f(a_1, \ldots, a_n)$ in $e_b$ gets replaced by $\mathtt{fi\_r1}(a_1, \ldots, a_n, r1-1, \ldots rk)$.
\line(1,0){\textwidth}\\

%& \lstinline|  requires q;|\\
%  $\fun f (x_1, \dots , x_n) = \{\cdots ; U_i; \cdots\}$ & \lstinline|  ensures p;|\\
%  $U_i = \hoare{Q}\mathbf (r_1 = (e_{min_1}, e_{len_1}), \hoare{I_{r1}}; $  & \lstinline|pure t fi(int x1, ..., int xn) =|
%  \\
%  \hspace{2em} $\cdots ; r_n = (e_{min_n}, e_{len_n}), \hoare{I_{r_{n}}}) \mathbf{~in~ }$ & \lstinline|  x1 == e1 && ... && xk == en && ep ? eb | \\
%  \hspace{2em} $(e_1, \ldots , e_n) \leftarrow e \mathbf{~if~} e_P \hoare{P}$ & \lstinline|    : fprev(x1, ..., xk)|\\
%  & where $t = \toT{U_0}$, $e1= \toE{e_1}$, ... , $ek= \toE{e_k}$, $eb = \toE{e_b}$,\\ & $ep = \toE{e_p}$, $q = \toE{Q}$, $p = \toE{P}$  and $fprev$ is the previous \\ & function stage. E.g. when defining $f4$ the previous \\
%  & stage is $f3$.\\ \hline


\centering
%\begin{tabular}{l@{\hspace{1em}}l}
%\hline
%Whole function transformation & \\
%$\fun f (x_1, \dots , x_n) = \{U_0; \cdots U_k \}$ & \lstinline|pure t f(int x1, ..., int xn) = fk(x1, ..., xn)|
%\\
% & where $t = \toT{U_0}$ \\ \hline
%Pure definition transformation & \lstinline|  requires q;| \\
%$\fun f (x_1, \dots , x_n) = \{U_0; \cdots U_k \}$ & \lstinline|  ensures p;| \\
% $U_0 = \hoare{Q}e\hoare{P}$ & \lstinline|pure t f0(int x1, ..., int xn) = e0;|\\
%
% & where $t = \toT{U_0}$, $e0 = \toE{e}$, $q = \toE{Q}$ and $p = \toE{P}$ \\ \hline
%%
%%
% Update definition (Empty reduction domain) & \lstinline|  requires q;|\\
% $\fun f (x_1, \dots , x_n) = \{\cdots ; U_i; \cdots\}$ & \lstinline|  ensures p;|\\
% $U_i = \hoare{Q}\rdom{} (e_1, \ldots , e_n) \leftarrow e \mathbf{~if~} e_P \hoare{P}$  & \lstinline|pure t fi(int x1, ..., int xn) =|
% \\
% & \lstinline|  x1 == e1 && ... && xk == en && ep ? eb | \\
% & \lstinline|    : fprev(x1, ..., xk)|\\
% & where $t = \toT{U_0}$, $e1= \toE{e_1}$, ... , $ek= \toE{e_k}$, $eb = \toE{e_b}$,\\ & $ep = \toE{e_p}$, $q = \toE{Q}$, $p = \toE{P}$  and $fprev$ is the previous \\ & function stage. E.g. when defining $f4$ the previous \\
% & stage is $f3$.\\ \hline
%%
%%
% Update definition (with reduction domain) & \lstinline|  requires q;|\\
%  $\fun f (x_1, \dots , x_n) = \{\cdots ; U_i; \cdots\}$ & \lstinline|  ensures p;|\\
%  $U_i = \hoare{Q}\mathbf (r_1 = (e_{min_1}, e_{len_1}), \hoare{I_{r1}}; $  & \lstinline|pure t fi(int x1, ..., int xn) =|
%  \\
%  \hspace{2em} $\cdots ; r_n = (e_{min_n}, e_{len_n}), \hoare{I_{r_{n}}}) \mathbf{~in~ }$ & \lstinline|  x1 == e1 && ... && xk == en && ep ? eb | \\
%  \hspace{2em} $(e_1, \ldots , e_n) \leftarrow e \mathbf{~if~} e_P \hoare{P}$ & \lstinline|    : fprev(x1, ..., xk)|\\
%  & where $t = \toT{U_0}$, $e1= \toE{e_1}$, ... , $ek= \toE{e_k}$, $eb = \toE{e_b}$,\\ & $ep = \toE{e_p}$, $q = \toE{Q}$, $p = \toE{P}$  and $fprev$ is the previous \\ & function stage. E.g. when defining $f4$ the previous \\
%  & stage is $f3$.\\ \hline
%\end{tabular}
\caption{\label{fig:translate} Rules for translating Halide algorithm code towards PVL.}
\end{figure}


We can translate the following piece of Halide code.
\begin{lstlisting}
Func blur(Buffer<int> input){
  Var x, y;
  Func blur_x, blur_y;
  Rdom r(-1,3, -1,3);
  input.requires(\result >= 0 && \result <= 255);

  blur(x,y) = 0;
  blur(x,y) += input(x+r.x,y+r.y);
  blur.invariant(r.x, \result >= 0 && \result <= 255 * ((r.y+1)*3+r.x+1));
  blur.invariant(r.y, \result >= 0 && \result <= 255 * (r.y+1)*3);
  blur(x,y) = blur(x,y)/9;
  blur.ensures(\result >= 0 && \result <= 255);

  return blur;
}
\end{lstlisting}

This gets translated to the PVL code below.
\begin{lstlisting}
  ensures \result >= 0 && \result <= 255;
pure int input(int x, int y);

pure int blur0(int x, int y) = 0;

pure int blur1(int x, int y) = blur1_ry(x,y,2);

  requires -1<=ry && ry<=2;
  ensures \result >= 0 && \result <= 255 * (r.y+1)*3;
pure int blur1_ry(int x, int y, int ry) =
  ry == -1 ? blur0(x, y) : blur1_rx(x, y, 2, ry-1)

  requires -1<=rx && rx<=2;
  requires -1<=ry && ry<2;
  ensures \result >= 0 && \result <= 255 * ((r.y+1)*3+r.x+1);
pure int blur1_rx(int x, int y, int rx, int ry) =
  rx == -1 && ry == -1 ? blur0(x, y)
    : rx == -1 ? blur1_rx(x, y, 2, ry-1)
      : blur1_rx(x, y, rx-1, ry) + input(rx-1, ry);

  ensures \result >= 0 && \result <= 255;
pure int blur2(int x, int y) = blur1(x,y)/9;

pure int blur(int x, int y) = blur2(x, y);
\end{lstlisting}
Note that since the update definitions of \lstinline|blur| the arguments are the same as in the pure definition (thus $x_1 = e_1 \wedge \cdots \wedge x_n = e_n$), thus we always go straight to the body statements, and skip an if-then-else check that is present in Fig. \ref{fig:translate} for the update definition. (We always get the $e_b$ path in our example).



\subsubsection{Limitations}
% Limitations
\begin{enumerate}
\item Invariants are needed for the lowest reduction variables, to prove anything correct. (The other invariants are not needed here, but are needed if we want to check the back-end).
\end{enumerate}

\subsection{Generating \& Transforming Annotations}\label{sec:transforming}
%Memory safety annotations

% Transforming Annotations with scheduling directives

% Limitations
